Sentiment Overflow in the Testing Stack: Analysing Software Testing Posts on Stack Overflow

Software testing is an integral part of modern software engineering practice. Past research has not only underlined its significance, but also revealed its multi-faceted nature. The practice of software testing and its adoption is influenced by many factors that go beyond tools or technology. This paper sets out to investigate the context of software testing from the practitioners' point of view by mining and analyzing sentimental posts on the widely used question and answer website Stack Overflow. By qualitatively analyzing sentimental expressions of practitioners, which we extract from the Stack Overflow dataset using sentiment analysis tools, we discern factors that help us to better understand the lived experience of software engineers with regards to software testing. Grounded in the data that we have analyzed, we argue that sentiments like insecurity, despair and aspiration, have an impact on practitioners' attitude towards testing. We suggest that they are connected to concrete factors like the level of complexity of projects in which software testing is practiced.

==> acks.tex <==
%! TEX root = paper.tex
\begin{acks}
This research was partially funded by the Dutch science foundation NWO through the Vici ``TestShift'' grant (No. VI.C.182.032).
\end{acks}


==> ccs.tex <==
% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
\begin{CCSXML}
\end{CCSXML}

\ccsdesc[300]{Software and its engineering~Programming teams}
\ccsdesc[300]{Human-centered computing~Natural language interfaces}
\ccsdesc[100]{Social and professional topics~Cultural characteristics}
\ccsdesc[100]{Computing methodologies~Simulation evaluation}


